It is Simple Sometimes: A Study On Improving Aspect-Based Sentiment Analysis Performance

Aspect-Based Sentiment Analysis (ABSA) involves extracting opinions from textual data about specific entities and their corresponding aspects through various complementary subtasks. Several prior research has focused on developing ad hoc designs of varying complexities for these subtasks. In this paper, we present a generative framework extensible to any ABSA subtask. We build upon the instruction tuned model proposed by Scaria et al. (2023), who present an instruction-based model with task descriptions followed by in-context examples on ABSA subtasks. We propose PFInstruct, an extension to this instruction learning paradigm by appending an NLP-related task prefix to the task description. This simple approach leads to improved performance across all tested SemEval subtasks, surpassing previous state-of-the-art (SOTA) on the ATE subtask (Rest14) by +3.28 F1-score, and on the AOOE subtask by an average of +5.43 F1-score across SemEval datasets. Furthermore, we explore the impact of the prefix-enhanced prompt quality on the ABSA subtasks and find that even a noisy prefix enhances model performance compared to the baseline. Our method also achieves competitive results on a biomedical domain dataset (ERSA).

==> app_extended_results.tex <==

% Table~\ref{tab:appcross-domain} provides extended results on the out-of-domain experiements.


% \begin{table}[]
% \centering
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{lccccc}
% \toprule
% Train& Test& Model &ATE &ATSC &AOOE \\ \midrule
% % \multirow{6}{*}{Lapt14} & \multirow{2}{*}{Rest14} & InstructABSA2 & & 83.13 & 80.28 \\ 
% % ~& ~& Ours-RE & & \textbf{82.75} & \textbf{84.89} \\ %85.58 \\ 
% % ~& \multirow{2}{*}{Rest15} & InstructABSA2 & & 84.87 & 87.01 \\ 
% % ~& ~& Ours-RE & & \textbf{85.42} & 86.12 \\ 
% % ~& \multirow{2}{*}{Rest16} & InstructABSA2 & & 85.20 & 83.66 \\ 
% % ~& ~& Ours-RE & & \textbf{83.90} & 89.21 \\ 
% % \midrule
% \multirow{2}{*}{Rest14} & \multirow{2}{*}{Lapt14} & InstructABSA2 & & \textbf{82.44}$^\dagger$ & 77.53 \\
% ~& ~& Ours-RE & & 80.38 & \textbf{87.06} \\ 
% \midrule
% \multirow{2}{*}{Rest15} & \multirow{2}{*}{Hotel15} & InstructABSA2 & & 89.74$^\dagger$ & - \\ 
% ~& ~& Ours-RE & & \textbf{91.16} & - \\ \midrule
% \multirow{4}{*}{Rest*} & \multirow{2}{*}{Lapt14} & InstructABSA2 & & 80.25 &77.53 \\ 
% ~& ~& Ours-RE & & \textbf{81.16} & 87.56 \\ 
% ~ & \multirow{2}{*}{Hotel15} & InstructABSA2 & &\textbf{92.56} & - \\ 
% ~& ~& Ours-RE & & 92.09 & - \\ 
% \bottomrule
% \end{tabular}
% }
% \caption{F1-scores for out-of-domain evaluation. Rest* stands for Restaurant domain, meaning that we trained the models jointly on Rest14, Rest15 and Rest16. $^\dagger$Results from original paper.}
% \label{tab:appcross-domain}
% \end{table}
% theirs: slurm-2264.out

% \section{Joint domain evaluation}

% To further validate our approach, we run an evaluation on a joint domain setting as done in \cite{scaria2023instructabsa}. In this setting, we train the model  
% Table~\ref{tab:appjoint} presents results for joint domain settings. 
% \begin{table}[]
% \centering
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{lccc}
% \toprule
% Model& Test& ATE &ATSC &AOOE \\ \midrule
% InstructABSA2& \multirow{2}{*}{Lapt14} &\textbf{83.60}$^\dagger$ &78.08 \\
% Ours-RE& ~&82.89 &85.28 \\ \midrule
% InstructABSA2& \multirow{2}{*}{Rest14} &88.03$^\dagger$ &80.89 \\
% Ours-RE& ~&\textbf{89.00} &89.26 \\
% \bottomrule
% \end{tabular}
% }
% \caption{Results of joint-domain evaluation. A model is trained on both Lapt14 and Rest14 datasets and evaluated on the each test set individually. ($^\dagger$) are from \citet{scaria2023instructabsa}.}
% \label{tab:appjoint}
% \end{table}

